Pre-train, Prompt, and Predict: A Systematic Survey of Prompting Methods in Natural Language Processing

This paper surveys and organizes research works in a new paradigm in natural language processing, which we dub "prompt-based learning". Unlike traditional supervised learning, which trains a model to take in an input x and predict an output y as P(y|x), prompt-based learning is based on language models that model the probability of text directly. To use these models to perform prediction tasks, the original input x is modified using a template into a textual string prompt x' that has some unfilled slots, and then the language model is used to probabilistically fill the unfilled information to obtain a final string x, from which the final output y can be derived. This framework is powerful and attractive for a number of reasons: it allows the language model to be pre-trained on massive amounts of raw text, and by defining a new prompting function the model is able to perform few-shot or even zero-shot learning, adapting to new scenarios with few or no labeled data. In this paper we introduce the basics of this promising paradigm, describe a unified set of mathematical notations that can cover a wide variety of existing work, and organize existing work along several dimensions, e.g.the choice of pre-trained models, prompts, and tuning strategies. To make the field more accessible to interested beginners, we not only make a systematic review of existing works and a highly structured typology of prompt-based concepts, but also release other resources, e.g., a website http://pretrain.nlpedia.ai/ including constantly-updated survey, and paperlist.

==> section/pretrain_old.tex <==

\subsection{Attention Mask}
% \pfliu{\url{https://arxiv.org/pdf/1910.10683.pdf}: Figure 3.}
% \gn{I feel like it'd be simpler to combine this section and the following section. There's basically a deterministic mapping between the masking strategies and the training strategies, right?}\pfliu{It would be nice if we can merge these two subsections, but for some framework like prefix LM, its encoder uses fully-connected but decoder uses diagonally-connected mask, I feel like it's a little hard to describe these frameworks without introducing the concepts of attention mask. Another way is to completely not mention the concept of attention mask.}
Attention masking is a technique to control the types of information that may be referenced when making predictions of different tokens in a sequence in models that use attention \citep{bahdanau2014neural}, such as the popular Transformer architecture~\cite{vaswani2017attention}.
This masking is closely connected with the training objective for the model, and we will discuss these combinations in the following section.
% For example, given a sentence ``\texttt{This is a good movie}'', this will dictate how to calculate the hidden state of the word ``\texttt{good}'' with Transformer without using the \texttt{movie}'s information.
% This is useful when Transformer is applied to language models. 
In general, three main types of masks are used, which we illustrate in Fig.~\ref{fig:attn_mask} and describe below using the illustrative example of calculating the representation of the word ``\texttt{good}'' in the sentence ``\texttt{This is a good movie}'': 
% Researchers usually use attention mask

\paragraph{Fully-connected mask}
This mask allows for any pairwise interaction between position $i$ and $j$ of a sequence. Every output element depends on any input token, so the word ``good'' would be influenced by all of the other words in the sentence. One typical example is BERT~\cite{devlin-etal-2019-bert}.

\paragraph{Diagonally-connected mask} 
This mask limits each token with position $i$ to only attending its history tokens while future tokens are invisible. Examples include GPT3~\cite{brown2020language} and BART~\cite{lewis-etal-2020-bart}.

\paragraph{Mixture mask}  
This mask allows for a mixture of the above two. A portion of the output elements depends on any input tokens (including its future inputs), while the rest of the output elements can not see its future input tokens. Examples include UniLM family \cite{DBLP:conf/nips/00040WWLWGZH19,DBLP:conf/icml/Bao0WW0L0GP0H20}.
More corresponding cases can be found in Tab.~\ref{tab:pretrained-aspect}.






% (1) fully-connected
% (2) Auto-regressive

\subsection{Typical Architecture} \label{sec:typical-architecture}
Different combined choices of the above dimensions (corruption, objective, mask strategy) could result in diverse pre-training language model architectures shown in Fig.~\ref{fig:four-architecture} and Tab.~\ref{tab:four-architecture}.
We first introduce the vanilla version and then show how its definition was extended for richer applicable scenarios.

% We introduce four commonly-used ones and describe them by elaborating on how they are used for modeling one sequence $X$ and a pair of sequences $(X, Y)$.

% draw some highlight boxes




% \paragraph{Auto-regressive Language Model (AR)}
% \pfliu{Q: Left-to-right or Auto-regresssive?}
\subsubsection{Left-to-Right Language Model}
% \subsubsection{Original Definition}
% \paragraph{Left-to-right Language Model (L2R LM)}
Also known as the auto-regressive language model, which aims to predict the upcoming words or assign probabilities $P(x_1, \cdots, x_n)$ to a sequence of words $X = x_1, \cdots, x_n$ \cite{jurafskyspeech}.
The probability is commonly broken down using the chain rule in a left-to-right fashion: $P(x_1,\cdots,x_t) = P(x_1)  \times \cdots P(x_t|w_1\cdots w_{t-1})$.\footnote{Similarly, a right-to-left language model can predict preceding words based on the future context, such as $P(x_1|x_2,x_3)$.}
% \begin{align}
%     P(x_1,\cdots,x_t) = P(x_1)  \times \cdots P(x_t|w_1\cdots w_{t-1})
% \end{align}

% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table*}[!htbp]
  \centering \footnotesize
    \begin{tabular}{lcccccll}
    \toprule
    \multirow{2}[2]{*}{\textbf{LMs}} & \multicolumn{3}{c}{\textbf{X}} & \multicolumn{3}{c}{\textbf{Y}}  & \multirow{2}[2]{*}{\textbf{Application}}\\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
          & \textbf{Mask} & \textbf{Corrupt} & \textbf{Main Object} & \textbf{Mask} & \textbf{Corrupt} & \textbf{Main Object} \\
    \midrule
    L2R   &  Diagonally  & None  & SLM   & -  & -  & - & In-context\\
    Mask  & Fully & Mask  & CTR   & -     & -     & -  & NLU\\
    Prefix& Fully & Any   & CTR   & Diagonally  & None  & SLM & NLU \& NLG \\
    En-De & Fully & Any   & None$\dag$  & Diagonally  & None  & FTR/CRT & NLU \& NLG \\
    \bottomrule
    \end{tabular}%
    \caption{Typical architectures for pre-trained language models. $X$ and $Y$ represent text to be encoded and decoded, respectively. 
    \textbf{SLM}: Standard language model.
    \textbf{CTR}: Corrupted text recover.
    \textbf{FTR}: Full text Reconstruction.
    $\dag$: Encoder-decoder architecture usually applies objective functions to the decoder part (e.g, BART). ``In-context'': L2R-based pre-trained models, such as GPT2/3 can also be used for conditional text generation with  additional prompts under the in-context learning setting detailed in \S\ref{sec:in-context-learning}.}
      \label{tab:four-architecture}%
\end{table*}%

% \renewcommand\bcStyleTitre[1]{\large\textcolor{ttblue}{#1}}
% \begin{bclogo}[
%   couleur=bgblue,
%   arrondi=0,
%   logo=\bcbombe,
%   barre=none,
%   noborder=true]{Commom Programming Error}
% \itshape
% can rely on information from both the left 
% \end{bclogo}

% \begin{mdframed}[style=mystyle,frametitle=Example \& Applicable Scenario]
% The conceptually simple nature of L2R makes it a prime candidate for training giant pre-trained language models (hundred billions of parameters). Representative examples include GPT-3,  PanGu-$\alpha$, Ernie-3.
% Earlier works such as GPT-1/2, ELMo also use L2R LM.

% L2R-based pre-trained language models are also the popular backbone that prompt learning will adopt, especially in zero-shot \cite{xx} or few-shot learning setting \cite{xx}. 
% The reason is pre-training models are too large or not publicized (e.g., GPT-3), and fine-tuning pre-trained models are unavailable.
% Therefore, using prompts to elicit knowledge from pre-trained models in a low-resource setting become the focus.
% \end{mdframed}

\begin{myboxi}[Example \& Applicable Scenario]
The conceptually simple nature of left-to-right (L2R) language model makes it a prime candidate for training giant pre-trained language models (hundred billions of parameters). Representative examples include GPT-3,  PanGu-$\alpha$~\cite{zeng2021pangualpha}, Ernie-3~\cite{DBLP:journals/corr/abs-2107-02137}.
Earlier works such as GPT-1/2~\cite{Radford2018ImprovingLU} also use L2R language model.

L2R-based pre-trained language models are also the popular backbone that prompting method will adopt, especially in zero-shot \cite{petroni-etal-2019-language,Radford2019LanguageMA} or few-shot learning setting \cite{brown2020language}. 
The reason is that pre-training models are too large or not publicized (e.g., GPT-3), and fine-tuning pre-trained models are unavailable.
Therefore, using prompts to elicit knowledge from pre-trained models in a low-resource setting become the focus.
\end{myboxi}

% \begin{myboxii}[Web addresses in text]
% can rely on information from both the left 
% \end{myboxii}

% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table*}[!htb]
  \renewcommand\tabcolsep{4.2pt}
\renewcommand{\arraystretch}{1.3}
  \centering \scriptsize
  
  

    \begin{tabular}{lllllclllll}
    \toprule%
    \multirow{2}[4]{*}{\textbf{Family}} & \multirow{2}[4]{*}{\textbf{Models}} & \multirow{2}[4]{*}{\textbf{LM}} & \multicolumn{3}{c}{\textbf{Pretraining Tasks}} & \multicolumn{4}{c}{\textbf{Corruption}} & \multirow{2}[4]{*}{\textbf{Application}} \\
\cmidrule(lr){4-6} \cmidrule(lr){7-10}          &       &       & \textbf{Main} & \textbf{Auxiliary} & \textbf{Parallel} & \textbf{Mask}  &\textbf{Replace} & \textbf{Delete} & \textbf{Permute}  &  \\
    \midrule
    \multirow{3}[2]{*}{\textbf{GPT}} & GPT \citenumber{Radford2018ImprovingLU}  & L2R    & SLM   & -     & \XSolidBrush  & -     & -     & -     & -     & NLG \\
          & GPT-2 \citenumber{Radford2019LanguageMA}  & L2R    & SLM   & -     & \XSolidBrush   & -    & -     & -     & -     & NLG \\
          & GPT-3 \citenumber{brown2020language}  & L2R    & SLM   & -     & \XSolidBrush  & -  & -     & -     & -     & NLG \\
          & Codex \citenumber{chen2021evaluating}  & L2R    & SLM   & -     & \XSolidBrush  & -  & -     & -     & -     & NLG \\

          
    \midrule
    \multirow{1}[1]{*}{\textbf{ELMo}} & ELMo \citenumber{peters-etal-2018-deep}  & L2R    & SLM   & -     & \XSolidBrush  & -   & -     & -     & -     & NLU, NLG \\
        %   & Flair \cite{DBLP:conf/coling/AkbikBV18}  & L2R    & SLM   & -     & -   & -     & -     & -     & NLU, NLG \\
    \midrule
    \multirow{12}[2]{*}{\textbf{BERT}} & BERT \citenumber{devlin-etal-2019-bert}  & Mask  & CTR   & NSP   & \XSolidBrush  & Tok  & -     & -     & -     & NLU \\
          & RoBERTa \citenumber{Liu2019RoBERTaAR} & Mask  & CTR   & -    & \XSolidBrush   & Tok   & -     & -     & -     & NLU \\
          & SpanBERT \citenumber{joshi-etal-2020-spanbert} & Mask  & CTR   & -    & \XSolidBrush   & Span & -     & -     & -     & NLU \\
          & SciBERT \citenumber{beltagy-etal-2019-scibert} & Mask  & CTR   & NSP   & \XSolidBrush  & Tok   & -     & -     & -     & Sci-NLU \\
          & BioBERT \citenumber{10.1093/bioinformatics/btz682} & Mask  & CTR   & NSP  & \XSolidBrush   & Tok  & -     & -     & -     & Bio-NLU \\
          & ALBERT \citenumber{DBLP:conf/iclr/LanCGGSS20} & Mask  & CTR   & SOP  & \XSolidBrush   & Tok   & -     & -     & -     & mSent \\
          & FinBERT \citenumber{DBLP:conf/ijcai/0001HH0Z20} & Mask  & CTR   & \makecell[l]{CWP, SDS, \\ SDP, TPP} & \XSolidBrush  & Span & -     & -     & Sent  & Fin-NLU \\
          & VLBERT \citenumber{DBLP:conf/iclr/SuZCLLWD20} & Mask  & CTR   & IRP   & \Checkmark  & Tok, Region & -     & -     & -     & VLU \\
          & ViLBERT \citenumber{DBLP:conf/nips/LuBPL19} & Mask  & CTR   & IRP, LVA & \Checkmark  & Tok, Region  & -     & -     & -     & VLU \\
          & VideoBERT \citenumber{DBLP:conf/iccv/SunMV0S19} & Mask  & CTR   & LVA   & \Checkmark  & Tok, Frame   & -     & -     & -     & VLU \\
          & TaBERT \citenumber{DBLP:conf/acl/YinNYR20} & Mask  & CTR   & MCP & \Checkmark  & Tok, Column   & -    & -     & -     & Tab2Text \\
          & mBERT \citenumber{devlin-etal-2019-bert} & Mask  & CTR   & NSP   & \XSolidBrush  & Tok   & -     & -     & -     & XLU \\
          & TinyBERT \citenumber{DBLP:conf/emnlp/JiaoYSJCL0L20} & Mask  & CTR   & NSP  & \XSolidBrush   & Tok   & -     & -     & -     & XLU \\
    \midrule
    \multirow{5}[2]{*}{\textbf{ERNIE}} & ERNIE-T \citenumber{DBLP:conf/acl/ZhangHLJSL19} & Mask  & CTR   & NSP  & \XSolidBrush   & Tok, Entity & -     & -     & -     & NLU \\
          & ERNIE-B \citenumber{sun2019ernie} & Mask  & CTR   & -   & \XSolidBrush  & Tok,Entity, Phrase   & -     & -     & -     & NLU \\
          & ERNIE-NG \citenumber{DBLP:conf/naacl/XiaoLZSTWW21} & Mask  & CTR   & RTD  & \XSolidBrush   & N-gram    & Tok     & -     & -     & NLU \\
          & ERNIE-B2 \citenumber{DBLP:conf/aaai/SunWLFTWW20} & Mask  & CTR   & \makecell[l]{CWP,SDS,SOP,\\SDP,DRP,IRR}  & \XSolidBrush  & Entity, Phrase  & -     & -     & Sent  & NLU \\
          & ERNIE-M \citenumber{DBLP:journals/corr/abs-2012-15674} & LPM   & CTR   & -    & \Checkmark   & Tok  & -     & -     &       & XLU, XLG \\
          &ERNIE-B3 \citenumber{DBLP:journals/corr/abs-2107-02137} & Mask     & CTR     & SOP,SDP,UKTP  & \XSolidBrush     & Entity, Phrase    & -     & -     & -     &  NLU    \\ 
    \midrule 
    \multirow{2}[2]{*}{\textbf{BART}} & BART \citenumber{lewis-etal-2020-bart}  & En-De & FTR   & -    & \XSolidBrush   & Tok    & Span  & Tok   & Sent,Doc     & NLU, NLG \\
          & mBART \citenumber{DBLP:journals/tacl/LiuGGLEGLZ20} & En-De & FTR   & -    & \XSolidBrush   & Span   & -     & -     & Sent  & NLG \\
    \midrule
    \multirow{2}[2]{*}{\textbf{UniLM}} & UniLM1 \citenumber{DBLP:conf/nips/00040WWLWGZH19} & LPM   & SLM,CTR & NSP   & \XSolidBrush  & Tok    & -     & -     & -     & NLU, NLG \\
          & UniLM2 \citenumber{DBLP:conf/icml/Bao0WW0L0GP0H20} & LPM   & SLM,CTR & -  & \XSolidBrush     & Tok    & -     & -     & Tok   & NLU, NLG \\
    \midrule
    \multirow{3}[2]{*}{\textbf{T5}} & T5 \citenumber{JMLR:v21:20-074}    & En-De & CTR   & -   & \XSolidBrush    & -   & Span  & -     & -     & NLU, NLG \\
          & mT5 \citenumber{DBLP:conf/naacl/XueCRKASBR21}   & En-De & CTR   & -  & \XSolidBrush     & -    & Span  & -     & -     & XLU, XLG \\
          & mT6 \citenumber{DBLP:journals/corr/abs-2104-08692}   & En-De & CTR    & MT,TPSC,TSC  & \Checkmark     & -     & Span & -     & -     & XLU, XLG \\
          & ByT5 \citenumber{DBLP:journals/corr/abs-2105-13626}   & En-De & CTR   & -   & \XSolidBrush    & -     & byte-span & -     & -     & XLU, XLG \\
    \midrule
    \multirow{2}[2]{*}{\textbf{XLM}} & XLM \citenumber{lample2019cross}  & LPM   & CTR   & TLM  & \Checkmark     & Tok   & -     & -     & -     & XLU, XLG \\
          & XLM-R \citenumber{DBLP:conf/acl/ConneauKGCWGGOZ20} & Mask  & CTR   & -    & \XSolidBrush    & Tok    & -     & -     & -     & XLU \\
          & XLM-E \citenumber{DBLP:journals/corr/abs-2106-16138} & Mask  & CTR   &  MRTD,TRTD  & \XSolidBrush     & -    & Tok     & -     & -     & XLU, XLG \\
    \midrule
    \multirow{2}[2]{*}{\textbf{CPM}} & CPM1 \citenumber{DBLP:journals/corr/abs-2012-00413}  & L2R    & SLM   & -   & \XSolidBrush    & -   & -     & -     & -     & NLG \\
          & CPM2  \citenumber{DBLP:journals/corr/abs-2106-10715}  & En-De    & CTR   & -  & \XSolidBrush     & Span   & -     & -     & -     & NLU,NLG \\    
     \midrule   
    \multirow{7}[2]{*}{\textbf{Other}} & XLNet \citenumber{DBLP:conf/nips/YangDYCSL19} & L2R    & SLM   & -   & \XSolidBrush    & -    & -      &  -     & Tok   & NLU \\
          & PanGu-$\alpha$ \citenumber{zeng2021pangualpha} & L2R    & SLM   & -   & \XSolidBrush    & -     & -     & -     & -     & NLG \\
          & ELECTRA \citenumber{DBLP:conf/iclr/ClarkLLM20} & Mask & CTR   & RTD & \XSolidBrush        & Tok   & Tok     & -     & -     & NLU,NLG \\
          & KEPLER \citenumber{DBLP:journals/tacl/WangGZZLLT21} & Mask & CTR   & -   & \XSolidBrush       - & Tok   & -     & -     & -     & NLU,NLG \\
          & MASS \citenumber{DBLP:conf/icml/SongTQLL19}  & En-De & CTR   & -   & \XSolidBrush    & Span     & -     & -     & -     & NLG \\
          & PEGASUS \citenumber{DBLP:conf/icml/ZhangZSL20} & En-De & CTR   & - & \XSolidBrush        - & Tok, Sent   & -     & -     & -     & Summarization \\
        %   & MASS \cite{DBLP:journals/corr/abs-1905-02450} & En-De & CTR   &      - & Tok   & -     & -     & -     & NLG \\
          & M6 \citenumber{DBLP:journals/tacl/WangGZZLLT21} & En-De & CTR   & ITT,MTT  & \XSolidBrush     & Span   & -     & -     & -     & NLG \\
          
    \bottomrule
    \end{tabular}%
  \caption{
  %Add caption\weizhey{Add SLM (All NLP tasks are generation tasks paper)?}
  A detailed illustration of different pre-trained models characterized by the four aspects.  
  ``\textbf{Parallel}'' represents if parallel data has been used for pre-training.
  \textbf{NSP}: Next sentence prediction;
  \textbf{SOP}: Sentence order prediction;
  \textbf{CWP}: Capital word  prediction;
  \textbf{SDS}: Sentence deshuffing;
  \textbf{SDP}: Sentence distance prediction;
  \textbf{CVP}: Cell value recovery;
  \textbf{LVA}: Linguistic-visual alignment;
  \textbf{RTD}: Replaced token detection;
  \textbf{DRP}: Discourse relation prediction;
  \textbf{L2R}: Left-to-right language models.
  \textbf{LPM}: Left-to-right, prefix, mask language models.
  \textbf{APP.} represents the applicable scenario which corresponding models are advantageous in.
  \textbf{NLU/G}: Natural language understanding or generation tasks.
  \textbf{XLU/G}: Cross-lingual understanding or generation tasks.
  \textbf{VLU}: Visual-language understanding.
  \textbf{UKTP}: Universal Knowledge-Text Prediction.
  \texttt{Sci}, \texttt{Bio}, \texttt{Fin}, \texttt{K} represent scientific, biomedical, financial, and knowledge, respectively.
  \texttt{Tok}, \texttt{Sent}, \texttt{Doc} denote token, sentence and document, respectively.
  \texttt{Region}, \texttt{Frame} denote basic units of images and video respectively.
%   \texttt{Summ.} denotes \textit{Summarization}.
  }
  \label{tab:pretrained-aspect}%
\end{table*}%



% \noindent \paragraph{Example \& Applicable Scenario}
% The conceptually simple nature of L2R makes it a prime candidate for training giant pre-trained language models (hundred billions of parameters). Representative examples include GPT-3,  PanGu-$\alpha$, Ernie-3.
% Earlier works such as GPT-1/2, ELMo also use L2R LM.

% L2R-based pre-trained language models are also the popular backbone that prompt learning will adopt, especially in zero-shot \cite{xx} or few-shot learning setting \cite{xx}. 
% The reason is pre-training models are too large or not publicized (e.g., GPT-3), and fine-tuning pre-trained models are unavailable.
% Therefore, using prompts to elicit knowledge from pre-trained models in a low-resource setting become the focus.


% draw some highlight boxes
% what's this?
% \note{Certainly elsewhere my do allowance at. The address farther six hearted hundred towards husband. Strangers ye to he sometimes propriety in. She right plate seven has. Bed who perceive judgment did marianne.}
% \warning{Doubtful two bed way pleasure confined followed. Shew up ye away no eyes life or were this.}
% \important{Travelling alteration impression six all uncommonly. Chamber hearing inhabit joy highest private ask him our believe. Up nature valley do warmly. Entered of cordial do on no hearted.}


% The language model is eventually trained in the hope that it can better serve the downstream tasks.
However, although the left-to-right language model is strong enough in decoding future words, it is not the most suitable architecture for some downstream tasks.

\subsubsection{Mask Language Model}

The pre-trained language model is eventually trained in the hope that it can better serve the downstream tasks.
For tasks such as text classification without requiring decoding a word from the left to right, it's important to make full use of input information and represent them better. For example, the representation of an input word can rely on information from both the left and right contexts.
To this end, the original definition of the language model has been extended to  a bidirectional variant: \term{mask language model}~\cite{devlin-etal-2019-bert}, which aims to
predict masked text pieces based on surrounded context. For example, $P(x_2|x_1,x_3)$ represents the probability of the word $x_2$ given its surrounded words $x_1$ and $x_3$.

\begin{myboxi}[Example \& Applicable Scenario]
Representative pre-trained models using the mask language model include: BERT, ERNIE~\cite{DBLP:conf/acl/ZhangHLJSL19,sun2019ernie} and their a variety of variants.
%and its variants, Ernie and its variants.
In prompting methods, the mask language model is generally suitable for those NLU tasks (e.g., text classification, semantic matching extractive question answering), which are often relatively easy to be reformulated into a cloze problem, and this is consistent with the training objectives of the mask language model. Additionally, instead of mainly focusing on zero-shot and few-shot setting, fine-tuning mask language pre-trained models has also been largely explored in prompting methods.
\end{myboxi}

% \noindent \paragraph{Example \& Applicable Scenario}
% Representative pre-trained models using the mask language model include: BERT, ERNIE and their a variety of variants.
% %and its variants, Ernie and its variants.
% In prompt learning, the mask language model is generally suitable for those NLU tasks (e.g., text classification, semantic matching extractive question answering), which are often relatively easy to be reformulated into a cloze problem, and this is consistent with the training objectives of the mask language model. Additionally, instead of mainly focusing on zero-shot and few-shot setting, fine-tuning mask language pre-trained models has also been largely explored in prompt learning.
%with mask language models Support zero-shot, few-shot, full-data fine-tune scenes.

% mask language models can be adopted are generally applied to natural language understanding tasks, such as text classification, semantic matching extractive question answering.


\subsubsection{Prefix and Encoder-Decoder}

For conditional text generation tasks such as translation and summarization where an input text $X = x_1, \cdots, x_n$ is given and the goal is to generate target text $Y = y_1, \cdots, y_m$, we not only need the pre-trained model to have a strong decoding ability but also better encode the input text. For example, better use of information both from left and right context for the given source language in machine translation task.
To achieve this goal, two popular architectures are proposed, and the basic idea is (1) using an encoder with fully-connected mask to encode the source $X$ first and then (2) decode the target $Y$ auto-regressively (from the left to right).


\paragraph{Prefix Language Model}
The prefix language model is a  (usually Transformer-based) left-to-right language model to decode $Y$ conditioned on a prefixed sequence $X$, which is encoded by the \textit{same} Transformer but with the fully-connected mask.
Notably, to encourage the pre-trained model to learn more, the corrupted operations (e.g., masking a token) are usually applied to the text $X$.
%that makes input fully connected.



\paragraph{Encoder-decoder}
The encoder-decoder model is a (usually Transformer-based) left-to-right language model to decode $Y$ conditioned on a \textit{separate} encoder (parameters of the encoder and decoder are not shared) for text $X$ with the fully-visible mask. Similar to the prefix language model, diverse text corruption can be made w.r.t. the input $X$.
%uses two sets of parameters for

\begin{myboxi}[Example \& Applicable Scenario]

Prefix LMs have been explored in UniLM 1-2 \cite{DBLP:conf/nips/00040WWLWGZH19,DBLP:conf/icml/Bao0WW0L0GP0H20} and ERNIE-M~\cite{DBLP:journals/corr/abs-2012-15674} while encoder-decoder models are widely used in T5~\cite{JMLR:v21:20-074}, BART~\cite{lewis-etal-2020-bart}, MASS~\cite{DBLP:conf/icml/SongTQLL19} and their variants.

Pre-trained models with prefix LMs and encoder-decoder paradigms can be naturally used to text generation tasks with \cite{dou-etal-2021-gsum} or without \cite{yuan2021can,liu2021simcls} prompting input texts.
However, recently studies reveal that more other non-generation tasks, such as information extraction \cite{cui2021templatebased}, questions answering  \cite{khashabi-etal-2020-unifiedqa}, evaluation  \cite{yuan2021bartscore} could be reformulated into a generation problem by prompting inputs in an appropriate way.
Therefore, prompting methods (i) broaden the applicability of these generation-oriented pre-trained models, and (ii) blur the boundaries between different tasks.

\end{myboxi}

% \noindent \paragraph{Example \& Applicable Scenario}



% Prefix LMs have been explored in UniLM 1-2 and ERNIE-M while encoder-decoder models are widely used in T5, BART, MASS and their variants.

% Pre-trained models with prefix LMs and encoder-decoder can be naturally used to text generation tasks with \cite{xx} or without \cite{xx} prompting input texts.
% However, recently studies reveal that more other non-generation tasks, such as information extraction \cite{xx}, questions answering  \cite{xx}, evaluation  \cite{xx} could be reformulated into a generation problem by prompting inputs in an appropriate way.
% Therefore, prompt learning broadens the applicability of these generation-oriented pre-trained models. 

% which broadens the applicability of Prefix usually focus on text generation tasks though they are can also be applied to NLU tasks.

